On the role of confinement on solidification in pure materials and binary alloys

We use a phase-field model to study the effect of confinement on dendritic growth, in a pure material solidifying in an undercooled melt, and in the directional solidification of a dilute binary alloy. Specifically, we observe the effect of varying the vertical domain extent ($\delta$) on tip selection, by quantifying the dendrite tip velocity and curvature as a function of $\delta$, and other process parameters. As $\delta$ decreases, we find that the operating state of the dendrite tips becomes significantly affected by the presence of finite boundaries. For particular boundary conditions, we observe a switching of the growth state from 3-D to 2-D at very small $\delta$, in both the pure material and alloy. We demonstrate that results from the alloy model compare favorably with those from an experimental study investigating this effect.

==> Images/jpegfiles/play_movie_ppm <==
dir=movies.$$
\rm -rf $dir
mkdir $dir

for file in *.ppm; 
do 
	out=${file%.*}.gif
	convert $file $out

	mv $out $dir
#	rm $file;
done

cd $dir && /home/badri/sw/gifsicle-1.39/bin/gifsicle -m -o movie.gif `ls -1 *.gif | sort -n` && mv movie.gif .. && 
cd ..

rm *.ppm
\rm -rf $dir

